Joint Routing and STDMA-based Scheduling to Minimize Delays in Grid Wireless Sensor Networks

In this report, we study the issue of delay optimization and energy efficiency in grid wireless sensor networks (WSNs). We focus on STDMA (Spatial Reuse TDMA)) scheduling, where a predefined cycle is repeated, and where each node has fixed transmission opportunities during specific slots (defined by colors). We assume a STDMA algorithm that takes advantage of the regularity of grid topology to also provide a spatially periodic coloring ("tiling" of the same color pattern). In this setting, the key challenges are: 1) minimizing the average routing delay by ordering the slots in the cycle 2) being energy efficient. Our work follows two directions: first, the baseline performance is evaluated when nothing specific is done and the colors are randomly ordered in the STDMA cycle. Then, we propose a solution, ORCHID that deliberately constructs an efficient STDMA schedule. It proceeds in two steps. In the first step, ORCHID starts form a colored grid and builds a hierarchical routing based on these colors. In the second step, ORCHID builds a color ordering, by considering jointly both routing and scheduling so as to ensure that any node will reach a sink in a single STDMA cycle. We study the performance of these solutions by means of simulations and modeling. Results show the excellent performance of ORCHID in terms of delays and energy compared to a shortest path routing that uses the delay as a heuristic. We also present the adaptation of ORCHID to general networks under the SINR interference model.

==> rr-annex.tex <==
\subsection{Approximation}
%===========================
%\subsection{Annex}
%===============
We introduce the following approximations that we use in our model.

\begin{approximation}\label{approx:realdis}
Let us consider a set of nodes $N_0, \dots, N_k$ for $k$ a positive integer $>0$ where each node $N_i$ has coordinates $(x_i, y_i)$. We approximate the distance between $N_0$ and $N_k$ by $\sum_{i=1}^{i=k} (x_i-x_{i-1})$.\\
\end{approximation}
Indeed, let us consider Figure~\ref{fig-approx1}. 
The distance $D=\sum_{i=1}^{i=k} (x_i-x_{i-1})$ corresponds to the distance needed by $N_0$ to reach node $N_k'$ following the x-axis. Now, to reach node $Nç_k$, $N_0$ needs to traverse in addition the distance $\delta$. However, when the transmission range $n\rightarrow\infty$, $\delta$ becomes small compared to $D$.  






\begin{figure}[h!]
\centering
\includegraphics[width=2.7in]{approx1}
\caption{Figure illustrating Approximation~1.\label{fig-approx1}}
\end{figure}
\begin{comment}
We have:
\begin{eqnarray*}
distance(N_0,N_k) & = &\sum_{i=1}^{i=k}{distance(N_i,N_{i-1})} \\
		   & = &\sum_{i=1}^{i=k}{\sqrt{(x_i-x_{i-1})^2+(y_i-y_{i-1})^2}} 
		%   & = &\sum_{i=1}^{i=k} (x_i-x_{i-1}) + \delta
\end{eqnarray*}
When~$n\rightarrow\infty$, $\delta$ is too small compared to  
$\sum_{i=1}^{i=k} (x_i-x_{i-1})$. 
The distance between any node $N_0$ and any node $N_k$ for any integer $k>0$ is equal to the $\sum_{i=1}^{i=k}(distance(N_i,N_{i-1}))$ (see Figure~\ref{fig:approx1}). The distance between any two nodes $N_i$ of coordinates $(x_i,y_i)$ and $N_j$ of coordinates $(x_j,y_j)$ which is equal to $\sqrt{(x_j-x_i)^2-(y_j-y_i)^2}$. We approximate this distance by $(x_j-x_j)$. Hence, this approximation makes sense. 
\end{comment}
%\end{approximation}

%This approximation makes sense because for large values of $n$, the distance $\delta$ is negligible compared to the real distance $\sum_{i=1}^{i=k}(distance(N_i,N_{i-1}))$ (see Figure~\ref{fig:approx1}). Hence, it suffices for the node $N_0$ to reach the node $N_{k}'$ and then reach $N_k$ via $\delta$.



\begin{approximation}\label{approx:log}
Asymptotically $log(1-a) = -a + o(a)$ for $a \rightarrow 0$.
\end{approximation}

\begin{approximation}\label{approx:integral}
We use the two following asymptotic expressions:
\begin{equation*}
\sum_{u=0}^{n}{\sqrt{n^2-u^2}} = \frac{\pi n^2}{4} + O(n)
\end{equation*}
\begin{equation*}
\sum_{u=0}^{n}{u\sqrt{n^2-u^2}} = \frac{n^3}{3} + O(n^2)
\end{equation*}
\end{approximation}
Indeed, these are sum of (bounded) functions, respectively: non-decreasing 
and with one unique maximum (increasing then decreasing).
It is easy to bound them with integrals:

\begin{eqnarray*}
 (\int_0^n \sqrt{n^2-u^2}~\mathrm{d}u) -n  & \le & \sum_{u=0}^{n}{\sqrt{n^2-u^2}} \le (\int_0^n \sqrt{n^2-u^2}~\mathrm{d}u)+n   ~~(\mathrm{since}~\sqrt{n^2-u^2} \le n) \\
%\end{eqnarray*}
%\begin{eqnarray*}
( \int_0^n u\sqrt{n^2-u^2}~\mathrm{d}u) - 3 n^2 & \le & \sum_{u=0}^{n}{u\sqrt{n^2-u^2}} \le (\int_0^n u\sqrt{n^2-u^2}~\mathrm{d}u) + 3 n^2  ~~(\mathrm{since}~u\sqrt{n^2-u^2} \le n^2)
\end{eqnarray*}



%\begin{eqnarray*}
%\sum_{u=0}^{n}{u\sqrt{n^2-u^2}} & =  & \int_0^n u\sqrt{n^2-u^2}~\mathrm{d}u + o(n)\\ %\substack{n\righarrow\infty}\\
%& \simeq & \int_0^n u\sqrt{n^2-u^2}~\mathrm{d}u   \mathrm{~~~when~n\rightarrow %\infty}\\ 
%& = & \[  -\frac{1}{3}(n^2-u^2)^{\frac{3}{2}} \]_0^n \\
%& = & \frac{n^3}{3}
%\end{eqnarray*}
%\end{approximation}

%U_n\underset{n\to +\infty}{\longrightarrow} 0

